Catching drifting pebbles I. Enhanced pebble accretion efficiencies for eccentric planets

Coagulation theory predicts that micron-sized dust grains grow into pebbles which drift inward towards the star, when they reach sizes of mm-cm. When they cross the orbit of a planet, a fraction of these drifting pebbles will be accreted. In the pebble accretion mechanism, the combined effects of the planet's gravitational attraction and gas drag greatly increase the accretion rate. We calculate the pebble accretion efficiency $\varepsilon_{2D}$ -- the probability a pebble is accreted by the planet -- in the 2D limit (pebbles reside in the midplane). In particular, we investigate the dependence of $\varepsilon_{2D}$ on the planet eccentricity and its implications for planet formation models. We conduct N-body simulations to calculate the pebble accretion efficiency in both the local frame and the global frame. With the global method we investigate the pebble accretion efficiency when the planet is on an eccentric orbit. We find that the local and the global methods generally give consistent results. The efficiency increases with the planet's eccentricity once the relative velocity between the pebble and the planet is determined by the planet's eccentric velocity. At large eccentricities, however, the relative velocity becomes too large for pebble accretion. The efficiency then drops significantly and the accretion enters the ballistic regime. We present general expressions for $\varepsilon_{2D}$. Applying the obtained formula to the formation of a secondary planet, in resonance with an already-formed giant planet, we find that the embryo grows quickly due to its larger eccentricity. The maximum $\varepsilon_{2D}$ for a planet on an eccentric orbit is several times higher than for a planet on a circular orbit, but this increase gives the planet an important headstart and boosts its following mass growth.

==> compare.tex <==
\section{Circular pebble accretion}
In this section, we only consider the planet in a circular orbit ($e =0$).  The comparison simulations among different methods are conducted in \se{compare}, and the analytical fitting expression for pebble accretion efficiency is illustrated in \se{analy}. 
\subsection{Comparison between different approaches}
\label{sec:compare}
We conduct simulations among three different approaches and compare the pebble accretion efficiencies. These approaches include the local frame integration (Local) (Ormel2010), the global frame direct integration (Global-direct), and the global frame hybrid method combined with direct integration and strong coupling approximation (Global-hybird).  
 Three masses of planets with varying $\taus$ have been explored. We focus on the pebble accretion (settling) cases where typically $10^{-3} \lesssim \taus < 1$, but for the additional method comparison, the cases of $\taus \gtrsim 1$ (ballistic regime) have also been investigated.

The strong coupling approximation (SCA) is applied to particles with $\taus \leqslant 10^{-2}$. In \fg{diff}, we verify that results of the hybrid method  well match with the direct method for these low $\taus$ particles.  Moreover,  the Global-hybrid algorithm  significantly reduces the computational time. For instance, the hybrid integration of a $0.1 \Me$ planet accreting particles of $\taus =10^{-2}$ is $10$ times faster than that of the direct integration, and $50$ times faster for the case of $\taus =10^{-3}$.

We also find that in \fg{diff} results from the local frame and the global frame are generally in good agreement with each other from  the low to the intermediate mass planet ($10^{-3} \Me$ and  $0.1 \Me$). Only massive planet case ($10 \Me$) the efficiencies obtained from the local simulations are higher than the global simulations. 

There are two limitations mainly caused for this difference. 
First, within the local framework there is a risk of multiple counting particles. 
There are  two possible ways of accretion when particles drift inward and across the orbit of the planet. Some of them either enter into the Hill sphere and directly hit onto the planet, Some others just flyby during the encounters, but orbit within the co-orbital region and re-accrete onto the planet again after a synodical time ($t_{\rm syn} \sim  \Omega_{\rm p}^{-1} r_{\rm p }/\Delta r_{\rm co}$, and $\Delta r_{\rm co}$ is the width of the co-orbital region of the planet).      
 % Physically, particles would either be accreted by the planet directly  (back side hit), or they do not hit the planet during the first encounter but re-accrete  later from the front side of the planet \coadd{sentence unclear}. 
 We initially place particles from both sides of planet in the local frame simulations. The problem for this initialization is that it may count the same particle twice, in particular when the radial drift of the particle is too small compared to the effective accretion radius ($r_{\rm eff}$) within a synodical time ($v_{\rm r} t_{\rm syn} < r_{\rm eff}$). We estimate that the planet beyond a few Earth mass may overestimate the efficiency due to this multiple counting effect.      

The other reason is  the linearization in the local frame . In the local approach, we ignore the high order terms of $(\Delta r_{\rm p}/\rp)^n$ ($n \geq2$) in the particle's equation of the motion regarding to the fact that $\Delta r_{\rm p} \ll  \rp$, where $\Delta r_{\rm p}$ is the distance between the planet and the particle. But the integration domain (maximum $\Delta r_{\rm p}$ we consider there) is larger for a more massive planet. Thus, the condition of $\Delta r_{\rm p} \ll  \rp$ breaks and  this first order approximation  is inappropriate for massive planets.  To conclude, both effects are biased to large $\Mp$, and as a result, the local results overestimate $\epsilon$ in the high mass branch.

We also find in \fg{diff} that the local and the global simulations fail to match with each when $\taus$ becomes large.
The cases of  $\taus =10$ are given where the accretion is in the ballistic regime. Two approaches have very different results, and this mismatch increases with the planet mass. In such a situation, the particle's eccentricity is excited by the planet during the encounter. The eccentricity damping from the gas drag is much longer than the encounter time ($\simeq$ orbital time). However, only (unperturbed) circular pebbles are assumed in the local frame simulations, which is not appropriated in this large $\taus$ case any more. There is no problem for the global simulations since it traces the full motion of the particles. For the $\Mp = 10 \Me $ and $\taus =10$ case,  global simulation gives  zero efficiencies. This is because the particles behave like planetesimals: they get trapped into  resonance with the planet. In summary, the global and the local frame are mostly consistent with each other.  But the global simulation accurately deals  with  cases of high mass planet ($\Mp \gtrsim 1-10 \Me$) and large particles size ($\taus \gtrsim 1 $). \ccc{(perhaps you mentioned this before): do say here that it is very straightforward and physically clear to extent the global approach towards eccentric planets. For the local approach this is not so obvious!.} 

  

\subsection{Analytical expression}
\label{sec:analy}
\ccc{My suggestion is to move most of this stuff to the appendix. The final part where you discuss the fits can be merged with the Analysis section}
We find that in \fg{diff} the accretion efficiency is a decreasing function of  the pebble size and an increasing  function of the planet mass. For a given planet, it is able to accrete small size pebbles more efficiently than those of large sizes. For a preferred size of pebbles, a massive planet can accretes more than a less massive one. 

Here we use a physical order-of-magnitude argument to explain such correlations. The expression is obtained  by combining the analytical and simulation results.   
There are two key requirements for pebble accretion (see Ormel2017):
\begin{enumerate}
    \item The time pebble settle onto the planet is shorter than the encounter time,  $t_{\rm set} < t_{\rm enc}$. Thus, the pebble is able to settle onto the planet before the flyby. This criterion is also equivalently  interpreted as the gravitational deflection time is shorter than the gas-pebble coupling time,  $t_{g} < t_{\rm s}$. 
    \item The gas-pebble coupling time is shorter than the pebble-planet encounter time,   $t_{\rm s} < t_{\rm enc}$. Otherwise,  the gas drag is not important during this encounter. 
\end{enumerate}
 
The failure of either criterion indicates the accretion is not in the settling regime.  
When gravitational acceleration equals to the gas drag, the settling velocity for the particle approaching the planet is given by   $v_{\rm set} = (GM_{\rm p}/r_{\rm eff}^2)  t_{\rm s}$, where $r_{\rm eff}$ is the effective pebble accretion radius.  The settling time $t_{\rm set}  \simeq r_{\rm eff}/v_{\rm set}$. The bypass timescale during an encounter, $t_{\rm enc} \simeq r_{\rm eff}/\Delta v$,
where $\Delta v$ is the relative velocity between the planet and the pebble.   
Based on criterion (1), $r_{\rm eff}$ can be written as 
% the gravitational deflection time ($\Delta v/(GM_{\rm p}/r_{\rm eff}^2)$) is equal to the gas-pebble coupling time ($t_{\rm s}$),
   \begin{equation} 
   \reff \sim \sqrt{\frac{GM_p t_s}{\Delta v}}.
   \label{eq:reff1}
      \end{equation} 

 
For a circular orbit planet, the relative velocity is either the headwind velocity of disk gas, $v_{\rm hw} \simeq \eta \vk$, or the Keplerian shear velocity between the planet and the pebble, $ v_{\rm sh} \sim \Omegak \reff$. The circular pebble accretion can naturally classified into two regimes by the dominated velocity: the headwind regime (Bondi regime) or the shear regime (Hill regime). 
%We therefore rewrite \eq{reff1} as 
%       \begin{equation} 
%   \reff  \sim 
%   \begin{cases}
%	\sqrt{GM_p t_s/ \eta \vk}  & \mbox{when } \Delta v = v_{\rm hw};\\ 
%	 (2\taus/3)^{1/3} R_{\rm H}   & \mbox{when } \Delta v = v_{\rm sh},
 %    \label{eq:reff}
 %    \end{cases}
 %     \end{equation} 
%where $v_{\rm hw} = \sqrt{1 + 4\taus^2}/(1 + \taus^2) \eta \vk \simeq \eta \vk$ and $ v_{\rm sh} \sim 3 \Omegak \reff/2 =  0.7 (q\taus)^{1/3} \vk$.
      
In a coplane (2D) accretion case, the mass flux of pebbles accreted by the planet is given by 
\begin{equation} 
  \dot M_{\rm PA} = 2 \reff \Delta v \Sigmap \sim  2 \sqrt{GM_p t_s \Delta v} \Sigmap.
  \label{eq:mdotpeb}
\end{equation}
%The total mass flux of pebbles sweeping through the orbit of the planet is given by  
%  \begin{equation} 
%  \dot M_{\rm disk} = 2 \pi \rp v_{\rm r} \Sigmap = 4 \pi \rp \eta  \taus  \vk  \Sigmap/(1 + \tau_s^2),
%  \label{eq:mdotdisk}
% \end{equation} 
 %where $\Sigmap$ is the pebble surface density, and   $v_{\rm r} (= 2\taus \eta \vk /(1+ \taus^2)$) is the radial drift velocity of the pebble. 
 According to the definition, the pebble accretion efficiency for a circular planet is given by
\begin{equation}
  \epsilon_0 = \frac{\dot M_{\rm PA}}{\dot M_{\rm disk}} \sim \frac{   \sqrt{GM_p t_{\rm s} \Delta v} (1 + \taus^2)  }{2 \pi \taus  \eta  V_{\rm K} r }
\end{equation}
Based on our numerical results, we change the prefactors in these expressions and further distinguish between the headwind and the shear regimes:
\begin{equation}
%\begin{split}
\epsilon_0 =
  \begin{cases}
%  &   	\begin{array}{ll}
	\epsilon_{\rm 0,hw} = 0.30	  q^{1/2} \eta^{-1/2} \tau_s^{-1/2} & \mbox{when }  q \leq q_{\rm hw/sh };  \\ 
	\epsilon_{\rm 0,sh}= 0.25 q^{2/3} \eta^{-1} \tau_s^{-1/3}  & \mbox{when }  q>  q_{\rm hw/sh}.
%	\end{array}
  \end{cases}
%\end{split}
\label{eq:efficiency0}
\end{equation}
We have used dimensionless quantities to express the efficiency where 
 $q \equiv M_{ \rm p}/M_{\star}= 3\times 10^{-6} (\Mp /1 \Me)$ and the headwind prefactor $\eta \equiv v_{\rm hw}/v_{\rm K} = 10^{-3} (\vhw/30 \rm  \ m/s)$. The $(1+\taus^{2})$ term is neglected since we focus on particles with $\taus<1$.  

Because the shear velocity increases with the planet mass, we expect that the low-mass planet mass is in the headwind regime and the massive planet is in the shear regime. 
The transition mass ratio  ($q_{\rm hw/sh}$) between these two regime can be estimated when $\vhw= v_{\rm sh}$.  Including a numerically-obtained prefactor, we find $ q_{\rm hw/sh} = 3 \eta^3 \taus^{-1}$. Finally, we adopt a uniform expression for two regimes and enforce $\epsilon_0 \leqslant 1$.  The accretion efficiency then reads
    \begin{equation} 
   \epsilon_0 = \min \left[C \epsilon_{\rm 0,hw} + ( 1 -C)\epsilon_{\rm 0,sh},1\right]. 
  \end{equation}
  where $C=\exp \left[-0.68(q/q_{\rm hw/sh})^{5}\right]$. It provides a sharp transition at $q_{\rm hw/sh}$, and both ensures $ \epsilon_0= \epsilon_{\rm 0,hw}$ for $q<q_{\rm hw/sh}$ and $ \epsilon_0= \epsilon_{\rm 0,sh}$ for $q>q_{\rm hw/sh}$. 

In \fg{diff}, we find that the analytical expression (black lines) agrees with the simulation results quite well in both regimes. One exception is for large stokes number pebbles ($\taus \gtrsim 1$). This is because the accretion is not in the settling regime any more. For the high masse cases, the analytical expression matches better for the global simulations than the local simulations, which has been explained in \se{compare}.



  % \begin{split} 
 %\epsilon =  &\frac{\dot M_{\rm acc}}{\dot M_{\rm peb}} = \frac{   \sqrt{8GM_p t_s \Delta v} (1 + \tau_s^2) }{4 \pi r \eta V_{\rm K} \tau_s}\\= 
%&\left\{
%	\begin{array}{ll}
%	0.2	q^{2/3} \eta^{-1} \tau_s^{-1/3} (1 + \tau_s^2)  & \mbox{when } e < e_{\rm sh}; \\
%	0.225 \xi^{1/2}	e^{1/2} \eta^{-1} q^{1/2} \tau_s^{-1/2}  (1 + \tau_s^2) & \mbox{when  } e \geq e_{\rm sh}.
%	\end{array}
%\right
%.
%\end{split}




\begin{figure*}[tbh!]
      \includegraphics[scale=1.0, angle=0]{diffapproach.pdf}
      \caption{\ccc{There is still no caption. Actually, I suggest to (i) to enlarge the figure -- it is an important result; (ii) then add more points so that it is clear the fitting formula works really well; (iii) add error bars; (iv) get rid of the ugly pink background color; (v) label axes properly\ldots} } 
\label{fig:diff}
\end{figure*} 


\begin{table*}
    \centering
    \caption{Pebble accretion efficiency comparison  between different approaches. The planet is in a circular orbit, and the disk headwind velocity is set to be  $30 \rm \  m/s$.}
    \begin{tabular}{llllllllllll|}
        \hline
        \hline
         $M_{\rm p } $ ($ \rm M_{\oplus}$)  & $\taus$ &   \multicolumn{3}{c}{Pebble accretion efficiency  $\epsilon_{\rm PA}$}\\
                &    & Local  & Global-direct  & Global-hybrid \\
        \hline
        \hline
        
     
       
       
       
      
       
       $10^{-3}$ &  $10^{-3} $  &  $1.73 \times 10^{-2}$    &   & $1.73 \times 10^{-2}$   \\
        $10^{-3}$ &  $10^{-2.5} $  &  $ 9.63 \times 10^{-3}$    &$  $ &$ 9.65 \times 10^{-3}$  \\
       $10^{-3}$ &  $10^{-2} $  &  $ 5.31 \times 10^{-3}$    &$5.31 \times 10^{-3}$ &$ 5.35 \times 10^{-3}$  \\
       $10^{-3}$   &  $10^{-1.5} $  &  $2.71 \times 10^{-3}$   & $2.71 \times 10^{-3}$ & $2.71 \times 10^{-3}$ \\
       $10^{-3}$   &  $10^{-1} $  &  $1.43 \times 10^{-3}$   & $1.45 \times 10^{-3}$ & $1.45 \times 10^{-3}$ \\
       $10^{-3}$  & $10^{-0.5} $   &  $8.9 \times 10^{-4}$    & $8.8 \times 10^{-4}$  & $8.8 \times 10^{-4}$    \\
       $10^{-3}$  & $0.5 $   &  $8 \times 10^{-4}$    & $8 \times 10^{-4}$  & $8 \times 10^{-4}$    \\
       $10^{-3}$    & $1 $       &  $8 \times 10^{-4}$    &$8 \times 10^{-4}$ & $8 \times 10^{-4}$  \\
       $10^{-3}$    & $10^{0.5} $       &  $ 6.5 \times 10^{-4}$    &$6.4 \times 10^{-4}$ & $6.4 \times 10^{-4}$  \\
       $10^{-3}$  &     $10 $ &   $6.9 \times 10^{-4}$    &$6.7 \times 10^{-4}$ & $6.7 \times 10^{-4}$  \\
            
             \hline
                    
           
            $0.1$  & $10^{-3} $&   $0.132$    & $0.129$ & $0.129$  \\
            $0.1$  & $10^{-2.5} $&   $7.89 \times 10^{-2}$    & $7.84 \times 10^{-2}$ & $7.84 \times 10^{-2}$  \\
            $0.1$ &$10^{-2} $ & $5.10\times 10^{-2}$     & $5.10 \times 10^{-2}$ & $5.10 \times 10^{-2}$ \\
            $0.1$ &$10^{-1.5} $ & $3.42 \times 10^{-2}$     & $3.42 \times 10^{-2}$ & $3.42 \times 10^{-2}$ \\
            $0.1$ &   $10^{-1} $  & $2.29 \times 10^{-2}$  &$2.30 \times 10^{-2}$  & $2.30 \times 10^{-2}$\\
            $0.1$  &   $10^{-0.5} $ &  $1.49 \times 10^{-2}$  &$1.5 \times 10^{-2}$ & $1.5 \times 10^{-2}$  \\
            $0.1$  &   $0.5 $ &  $1.27 \times 10^{-2}$  &$1.27 \times 10^{-2}$ & $1.27 \times 10^{-2}$  \\
            $0.1$ &  $1 $ &   $7.85 \times 10^{-3}$ &$7.80 \times 10^{-3}$ & $7.80 \times 10^{-3}$  \\
            $0.1$ &  $10^{0.5} $ &   $9.83 \times 10^{-3}$ &$9.65 \times 10^{-3}$ & $9.65 \times 10^{-3}$  \\
            $0.1$  & $1 0$   &  $2.67\times 10^{-2}$   &$1.37 \times 10^{-2}$ & $1.37 \times 10^{-2}$ \\

          \hline
              
                 $10$  &    $10^{-3} $&   $2.83$    & $1.0$ & $1.0$  \\
                 $10$  &   $10^{-2.5} $&   $1.93$   & $0.96$ & $0.95$ \\
                 $10$  &   $10^{-2} $&   $1.25$   & $0.75$ & $0.75$ \\
                 $10$  &$10^{-1.5} $ &  $0.83$ &$0.57$  & $0.57$ \\
                 $10$  &$10^{-1} $ &  $0.53$ &$0.45$  & $0.45$ \\
                 $10$ &$0.5 $ &  $0.27$  &$0.24$ &  $0.24$ \\
                 $10$ &$10^{-0.5} $ &  $0.331$  &$0.284$ &  $0.284$ \\
                 $10$  &  $1 $   &   $0.23$ &$0.13$ & $0.13$ \\
                 $10$  &  $10^{0.5} $   &   $0.386$ &$0.195$ & $0.195$ \\
                 $10$ &$10$ &  $0.58$   &$0$ &$0$&  \\


          \hline
        \hline
    \end{tabular}
    \label{tab:tab1}
\end{table*}



%\begin{table*}
%    \centering
%    \caption{Comparison of the pebble accretion efficiency  between different approaches. The planet is in a circular orbit, and the disk headwind velocity is set as  $30 \rm \  m/s$.}
%    \begin{tabular}{llllllllllll|}
%        \hline
%        \hline
%        Run  & $\taus$ & $M_{\rm p } $ ($ \rm M_{\oplus}$)     & \multicolumn{3}{c}{Pebble accretion efficiency  $\epsilon_{\rm PA}$}\\
%                &    &      & Local  & Global\footnote[1]{ without optimized algorithm}  & Global -SCA \\
%        \hline
     
% \#1& $10 $      & $10^{-3}$  & $6.9 \times 10^{-4}$    &$6.7 \times 10^{-4}$ &  \\
%    \#2& $1 $      & $10^{-3}$  &  $8 \times 10^{-4}$    &$8 \times 10^{-4}$ &  \\
%     \#3& $0.5 $      & $10^{-3}$  &  $8 \times 10^{-4}$    & $8 \times 10^{-4}$  &   \\
%     \#4& $10^{-1} $      & $10^{-3}$  &  $1.43 \times 10^{-3}$   & $1.45 \times 10^{-3}$ \\
%     \#5& $10^{-2} $      & $10^{-3}$  &  $ 5.31 \times 10^{-3}$    &$5.31 \times 10^{-5}$ &$ 5.35 \times 10^{-3}$  \\
%     \#6& $10^{-3} $      & $10^{-3}$  &  $1.73 \times 10^{-2}$    &   & $1.73 \times 10^{-2}$   \\
%      \#7& $10 $      & $1$  &   $6.23 \times 10^{-2}$    &$5.98 \times 10^{-2}$ &  \\
%      \#8& $1 $      & $1$  &  $3.24 \times 10^{-2}$    &$3.22 \times 10^{-2}$ &  \\
%       \#9& $0.5 $      & $1$  &  $5.64 \times 10^{-2}$    &$5.66 \times 10^{-2}$ &  \\
%       \#10& $10^{-1} $      & $1$ & $0.10$ &   $0.10$  &\\
%       \#11& $10^{-2} $      & $1$  &  $0.19$      &  $0.22$ & $0.22$ \\
%       \#12& $10^{-3} $      & $1$  &  $0.43$      & $0.44$ & $0.43$  \\
       
%       \#13& $1 0$      & $0.1$  &  $2.67\times 10^{-2}$   &$1.37 \times 10^{-2}$ &  \\
%        \#14& $1 $      & $0.1$  &   $7.85 \times 10^{-3}$ &$7.80 \times 10^{-3}$ &  \\
%       \#15& $0.5 $      & $0.1$  &  $1.27 \times 10^{-2}$  &$1.27 \times 10^{-2}$ &  \\
%       \#16& $10^{-1} $      & $0.1$  & $2.29 \times 10^{-2}$  &$2.30 \times 10^{-2}$  &\\
%       \#17& $10^{-2} $      & $0.1$  & $5.1\times 10^{-2}$     &  & $5.1 \times 10^{-2}$ \\
  %     \#18& $10^{-3} $      & $0.1$  &   $0.132$    & $$ & $0.129$  \\
       
              
  %     \#19& $1 0$      & $10$  &  $0.58$   &$<2\times 10^{-3}$ &  \\
  %      \#20& $1 $      & $10$  &   $0.23$ &$0.13$ &  \\
  %     \#21& $0.5 $      & $10$  &  $0.27$  &$0.24$ &  \\
  %     \#22& $10^{-1} $      & $10$  &  $0.53$ &$0.45$  &\\
  %     \#23& $10^{-2} $      & $10$  &    $1.25$   &  & $0.75$ \\
  %     \#24& $10^{-3} $      & $10$  &   $2.83$    & $$ & $1.0$  \\

  %        \hline
  %      \hline
  %  \end{tabular}
  %  \label{tab:tab1}
%\end{table*}

